Supervised Fitting of Geometric Primitives to 3D Point Clouds

Fitting geometric primitives to 3D point cloud data bridges a gap between low-level digitized 3D data and high-level structural information on the underlying 3D shapes. As such, it enables many downstream applications in 3D data processing. For a long time, RANSAC-based methods have been the gold standard for such primitive fitting problems, but they require careful per-input parameter tuning and thus do not scale well for large datasets with diverse shapes. In this work, we introduce Supervised Primitive Fitting Network (SPFN), an end-to-end neural network that can robustly detect a varying number of primitives at different scales without any user control. The network is supervised using ground truth primitive surfaces and primitive membership for the input points. Instead of directly predicting the primitives, our architecture first predicts per-point properties and then uses a differential model estimation module to compute the primitive type and parameters. We evaluate our approach on a novel benchmark of ANSI 3D mechanical component models and demonstrate a significant improvement over both the state-of-the-art RANSAC-based methods and the direct neural prediction.

==> sections/framework_orig.tex <==
% !TEX root = ../paper.tex

\section{Supervised Primitive Fitting Network}
\label{sec:framework}
\vspace{-3pt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t!]
  \includegraphics[width=\textwidth]{figures/pipeline.pdf}
\caption{Network architecture. PointNet++~\cite{Qi:2017b} takes input point cloud $\mathbf{P}$ and outputs three per-point properties: point-to-primitive membership $\mathbf{\hat{W}}$, normals $\mathbf{\hat{N}}$, and associated primitive type $\mathbf{\hat{T}}$. The order of ground truth primitives are matched with the output in the primitive reordering step (Section~\ref{sec:primitives_reordering}). Then, the output primitive parameters are estimated from the point properties in the model estimations step (Section~\ref{sec:model_estimation}). The loss is defined as the sum of five loss terms  (Section~\ref{sec:loss_function}).}
\label{fig:pipeline}
\vspace{-\baselineskip}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We propose Supervised Primitive Fitting Network (SPFN) that takes an input shape represented by a point cloud $\mathbf{P} \in \mathbb{R}^{N \times 3}$, where $N$ is number of points, and predicts a set of geometric primitives that best fit the input. 
The output of SPFN contains the type and parameters for every primitive, plus a list of input points assigned to it. 
Our network supports $L=4$ types of primitives: plane, sphere, cylinder, and cone (Figure~\ref{fig:primitives}), and we index these types by $0, 1, 2, 3$ accordingly.
Throughout the paper, we will use notations $\{\cdot\}_{i,:}$ and $\{\cdot\}_{:,k}$ to denote $i$-th row and $k$-th column of a matrix, respectively. 

During training, for each input shape with $K$ primitives, SPFN leverages the following ground truth information as supervision: point-to-primitive membership matrix $\mathbf{W} \in \{0, 1\}^{N\times K}$, unoriented point normals $\mathbf{N} \in \mathbb{R}^{N \times 3}$, and bounded primitive surfaces $\{\mathbf{S}_{k}\}_{k=1,\ldots, K}$. 
For the membership matrix, $\mathbf{W}_{i,k}$ indicates if point $i$ belongs to primitive $k$ so that $\sum_{k=1}^K \mathbf{W}_{i,k} \le 1$.
Notice that $\mathbf{W}_{:,k}$, the $k$-th column of $\mathbf{W}$, indicates the \emph{point segment} assigned to primitive $k$. 
We allow $K$ to \emph{vary} for each shape, and $\mathbf{W}$ can have zero rows indicating \emph{unassigned} points (points not belonging to any of the $K$ primitives; e.g. it belongs to a primitive of unknown type).
Each $\mathbf{S}_k$ contains information about the type, parameters, and boundary of the $k$-th primitive surface, and we denote its type by $\mathbf{t}_k \in \{0,1,\ldots, L-1\}$ and its type-specific parameters by $\mathbf{A}_k$.
We include the boundary of $\mathbf{S}_k$ in the supervision besides $\mathbf{P}$ because $\mathbf{P}$ can be noisy, and we do not discriminate against small surfaces in evaluating per-primitive losses (see Equation \ref{eq:residual_loss}).
For convenience, we define per-point type matrix $\mathbf{T} \in \{0, 1\}^{N \times L}$ by $\mathbf{T}_{i,l} = \sum_{k=1}^K \mathbb{1} (\mathbf{W}_{i,k}=1)\mathbb{1}(\mathbf{t}_k = l)$, where $\mathbb{1}(\cdot)$ is the indicator function.


The pipeline of SPFN at training time is illustrated in Figure~\ref{fig:pipeline}. We use PointNet++~\cite{Qi:2017b} segmentation architecture to consume the input point cloud $\mathbf{P}$. A slight modification is that we add three separate fully-connected layers to the end of the PointNet++ pipeline in order to predict the following per-point properties: point-to-primitive membership matrix $\mathbf{\hat{W}} \in [0, 1]^{N\times K}$\footnote{For notational clarity, for now we assume the number of predicted primitives equals $K$, the number of ground truth primitives. See Section \ref{sec:implementation_details} for how to predict $\mathbf{\hat W}$ without prior knowledge of $K$.}, unoriented point normals $\mathbf{\hat{N}} \in \mathbb{R}^{N \times 3}$, and per-point primitive types $\mathbf{\hat{T}} \in [0, 1]^{N\times L}$. We use softmax activation to obtain membership probabilities in the rows of $\mathbf{\hat{W}}$ and $\mathbf{\hat{T}}$, and we normalize the rows of the $\mathbf{\hat{N}}$ to constrain normals to have $l^2$-norm $1$. 
% In our convention, we use letters with hat to represent predicted quantities in contrast with their ground truth versions.
We then feed these per-point quantities to our \emph{differentiable model estimator} (Section \ref{sec:model_estimation}) that computes primitive parameters $\{\mathbf{\hat{A}}_k\}$ based on the per-point information. Since this last step is differentiable, we are able to backpropagate any kind of per-primitive loss through the PointNet++, and thus the training can be done end-to-end.
% the fitting residual loss can still be measured from points to the estimated models and backpropagated end-to-end.
%\AD{what does it mean that "the primitives are estimated"? How is this related to the "fitting residual loss"? We need a more clear explanation, and I'm not sure what it should be}.
% Layers outputting memberships and types  apply softmax activation to each row of the matrices, and a layer generating normals $\mathbf{\hat{N}}$ $l2$-normalizes each row.

% The prediction of the membership matrix $\mathbf{\hat{W}}$ differs from a standard classification problem in that the ground truth primitives have no consistent order across different shapes. 

Notice that we do not assume a consistent ordering of ground truth primitives, so we do not assume any ordering of the columns of our predicted $\mathbf{\hat{W}}$.
In Section~\ref{sec:primitives_reordering}, we describe the \emph{primitive reordering} step used to handle such mismatch of orderings. In Section~\ref{sec:model_estimation}, we present our differential model estimator for predicting primitive parameters $\{\mathbf{\hat{A}}_{k}\}$. In Section~\ref{sec:loss_function}, we define each term in our loss function. Lastly, in Section~\ref{sec:implementation_details}, we describe implementation details.


\subsection{Primitives Reordering}
\label{sec:primitives_reordering}
\vspace{-3pt}
% At the first stage, the predicted point-to-primitive memberships $\mathbf{\hat{W}}$ are used to reorder the ground truth primitives so that the corresponding ground truth and predicted primitives can be indexed jointly. 
Inspired by Yi \etal~\cite{Yi:2018}, we compute \emph{Relaxed Intersection over Union} (RIoU)~\cite{Krahenbuhl:2013} for all pairs of columns from the membership matrices $\mathbf{W}$ and $\mathbf{\hat{W}}$. The RIoU for two indicator vectors $\mathbf{w}$ and $\mathbf{\hat{w}}$ is defined as follows:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
\text{RIoU}(\mathbf{w}, \mathbf{\hat{w}}) = \frac{\mathbf{w}^\mathbf{T}\mathbf{\hat{w}}}{\|\mathbf{w}\|_1 + \|\mathbf{\hat{w}}\|_1 -  \mathbf{w}^\mathbf{T}\mathbf{\hat{w}}}.
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The best one-to-one correspondence (determined by RIoU) between columns of the two matrices is then given by Hungarian matching~\cite{Kuhn:1955}. 
We reorder the ground truth primitives according to this correspondence, so that ground truth primitive $k$ is matched with the predicted primitive $k$. 
%We remark that the Hungarian matching step in our framework can be considered as an inner discrete optimization in an alternating optimization scheme similarly to~\cite{Sung:2018}. 
%We recognize the set of inputs where a small perturbation will lead to a change of the correspondence has measure zero, so the overall pipeline remains differentiable.
Since the set of inputs where a small perturbation will lead to a change of the matching result has measure zero, the overall pipeline remains differentiable almost everywhere. Hence we use an external Hungarian matching solver to obtain optimal matching indices, and then inject these back into our network to allow further loss computation and gradient propagation.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t!]
\centering
\begin{minipage}[t]{.25\columnwidth}
  \includegraphics[width=\linewidth,trim={0.8cm 0.8cm 0.8cm 0.8cm},clip]{figures/primitives/plane.pdf}
\end{minipage}% 
\begin{minipage}[t]{.25\columnwidth}
  \includegraphics[width=\linewidth,trim={0.8cm 0.8cm 0.8cm 0.8cm},clip]{figures/primitives/sphere.pdf}
\end{minipage}% 
\begin{minipage}[t]{.25\columnwidth}
  \includegraphics[width=\linewidth,trim={0.8cm 0.8cm 0.8cm 0.8cm},clip]{figures/primitives/cylinder.pdf}
\end{minipage}% 
\begin{minipage}[t]{.25\columnwidth}
  \includegraphics[width=\linewidth,trim={0.8cm 0.8cm 0.8cm 0.8cm},clip]{figures/primitives/cone.pdf}
\end{minipage}
\vspace{-\baselineskip}
\caption{Primitive types and parameters. The boundary information in each  $\mathbf{S}_k$, together with parameters $\mathbf{A}_k$, defines the (bounded) region of the primitive $k$. On the other hand, the point segment $\mathbf{W}_{:,k}$ provides an approximation to this bounded region.}
\label{fig:primitives}
\vspace{-\baselineskip}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Primitive Model Estimation}
\label{sec:model_estimation}
\vspace{-3pt}
In the model estimation module, primitive parameters $\{\mathbf{A}_k\}$ are obtained from the predicted per-point properties in a differentiable manner. 
As the parameter estimation for each primitive is independent, in this section we will assume $k$ is a fixed index of a primitive.
The input to the model estimation module consists of $\mathbf{P}$, the input point cloud, $\mathbf{\hat{N}}$, the predicted unoriented point normals, and $\mathbf{\hat{W}}_{:,k}$, the $k$-th column of the predicted membership matrix $\mathbf{\hat{W}}$. For simplicity, we write $\mathbf{w} = \mathbf{\hat{W}}_{:,k} \in [0, 1]^N$ and $\mathbf{\hat{A}} = \mathbf{\hat{A}}_k$. 
For $\mathbf{p} \in \mathbb{R}^3$, let $D_{l}(\mathbf{p}, \mathbf{A})$ denote the distance from $\mathbf{p}$ to the primitive of type $l$ and parameters $\mathbf{A}$.
The differentiable module for computing $\mathbf{\hat{A}}$, given the primitive type, is illustrated below.

\vspace{-\baselineskip}
\paragraph{Plane.}
A plane is represented by $\mathbf{A} = (\mathbf{a}, d)$ where $\mathbf{a}$ is the normal of the plane, with $\| \mathbf{a} \| = 1$, and the points on the plane are $\{\mathbf{p} \in \mathbb{R}^3 : \mathbf{a}^{\mathbf{T}} \mathbf{p} = d\}$. Then
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
  D^2_{\text{plane}}(\mathbf{p}, \mathbf{A}) = (\mathbf{a}^{\mathbf{T}} \mathbf{p} - d)^2.
\label{eq:plane_residual}
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We can then define $\mathbf{\hat{A}}$ as the minimizer to the \emph{weighted} sum of squared distances as a function of $\mathbf{A}$:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
  \mathcal{E}_{\text{plane}}(\mathbf{A}; \mathbf{P}, \mathbf{w})
  &= \sum_{i=1}^N \mathbf{w}_i (\mathbf{a}^\mathbf{T} \mathbf{P}_{i,:} - d)^2.
  %&= \sum_{i=1}^N \mathbf{w}_i D^2_{\text{plane}}(\mathbf{P}_{i,:}, \mathbf{A}) \\
\label{eq:plane_weighted}
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
By solving $\frac{\partial \mathcal{E}_{\text{plane}}}{\partial d} = 0$, we obtain $d = \frac{\sum_{i=1}^N \mathbf{w}_i \mathbf{a}^\mathbf{T} \mathbf{P}_{i,:}}{\sum_{i=1}^N \mathbf{w}_i}$.
Plugging this into Equation~$\ref{eq:plane_weighted}$ gives:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
  \mathcal{E}_{\text{plane}}(\mathbf{a}; \mathbf{P}, \mathbf{w}) = \norm{\text{diag}\left(\mathbf{w}\right) \mathbf{X} \mathbf{a}}^2,
\label{eq:plane_weighted_axis}
\end{equation}
where $\mathbf{X}_{i,:} = \mathbf{P}_{i,:} - \textstyle\frac{\sum_{i=1}^N \mathbf{w}_i \mathbf{P}_{i,:}}{\sum_{i=1}^N \mathbf{w}_i}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Hence minimizing $\mathcal{E}_{\text{plane}}(\mathbf{A}; \mathbf{P}, \mathbf{w})$ over $\mathbf{a}$ becomes a homogeneous least square problem subject to $\| \mathbf{a} \| = 1$, and its solution is given as the right singular vector $\mathbf{v}$ corresponding to the smallest singular value of matrix $\text{diag}\left(\mathbf{w}\right) \mathbf{X}$. As shown by Ionescu~\etal~\cite{Ionescu:2015a,Ionescu:2015b}, the gradient with respect to $\mathbf{v}$ can be backpropagated through the SVD computation.

\vspace{-\baselineskip}
\paragraph{Sphere.}
A sphere is parameterized by $\mathbf{A} = (\mathbf{c}, r)$, where $\mathbf{c} \in \mathbb{R}^3$ is the center and $r \in \mathbb{R}$ is the radius. Hence
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
  D^2_{\text{sphere}}(\mathbf{p}, \mathbf{A}) = (\norm{\mathbf{p} - \mathbf{c}} - r)^2
.\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In the sphere case (also in the cases of cylinder and cone), the squared distance is not quadratic. Hence minimizing the weighted sum of squared distances over parameters as done in the plane is only available via nonlinear iterative solvers~\cite{Lukacs:1998}. Instead, we consider minimizing over the weighted sum of a different notion of distance:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
  \mathcal{E}_{\text{sphere}}(\mathbf{A}; \mathbf{P}, \mathbf{w}) = \sum_{i=1}^N \mathbf{w}_i (\norm{\mathbf{P}_{i,:} - \mathbf{c}}^2 -r^2)^2.
  \label{eq:sphere_weighted}
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Solving $\frac{\partial \mathcal{E}_{\text{sphere}}}{\partial r^2} = 0$ gives $r^2 = \frac{1}{\sum_{i=1}^N \mathbf{w}_i} \sum_{j=1}^N\mathbf{w}_j \|\mathbf{P}_j - \mathbf{c}\|^2$. 
Putting this back in Equation \ref{eq:sphere_weighted}, we end up with a quadratic expression in $\mathbf{c}$ as a least square:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
  \mathcal{E}_{\text{sphere}}(\mathbf{c}; \mathbf{P}, \mathbf{w}, \mathbf{a}) = \norm{\text{diag}\left(\mathbf{w}\right) (\mathbf{X}\mathbf{c} -\mathbf{y})}^2,
\label{eq:sphere_weighted_center}
\end{equation}
where $\mathbf{X}_{i,:} = 2\left(-\mathbf{P}_{i,:} + \textstyle\frac{\sum_{j=1}^N \mathbf{w}_j \mathbf{P}_{j,:}}{\sum_{j=1}^N \mathbf{w}_j}\right)$ and
$\mathbf{y}_{i} = \mathbf{P}_{i,:}^{\mathbf{T}}\mathbf{P}_{i,:} - \textstyle\frac{\sum_{j=1}^N \mathbf{w}_j \mathbf{P}_{j,:}^{\mathbf{T}}\mathbf{P}_{j,:}}{\sum_{j=1}^N \mathbf{w}_j}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
This least square can be solved via Cholesky factorization in a differentiable way~\cite{Murray:2016}.

\vspace{-\baselineskip}
\paragraph{Cylinder.}
A cylinder is parameterized by $\mathbf{A} = (\mathbf{a}, \mathbf{c}, r)$ where $\mathbf{a} \in \mathbb{R}^3$ is a unit vector of the axis, $\mathbf{c} \in \mathbb{R}^3$ is the center, and $r \in \mathbb{R}$ is the radius. We have
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
  D^2_{\text{cylinder}}(\mathbf{p}, \mathbf{A}) = \left( \sqrt{\mathbf{v}^{\mathbf{T}}\mathbf{v} - (\mathbf{a}^{\mathbf{T}}\mathbf{v})^2} - r \right)^2,
\end{equation}
where $\mathbf{v} = \mathbf{p} - \mathbf{c}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
As in the sphere case, directly minimizing over squared true distance is challenging. Instead, inspired by Nurunnabi et. al.~\cite{Nurunnabi:2017}, we first estimate the axis $\mathbf{a}$ and then solve a circle fitting to obtain the rest of the parameters.
Observe that the normals of points on the cylinder must be perpendicular to $\mathbf{a}$, so we choose $\mathbf{a}$ to minimize:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
  \mathcal{E}_{\text{cylinder}}(\mathbf{a}; \mathbf{\hat{N}}, \mathbf{w}) = \norm{ \text{diag}\left(\mathbf{w}\right) \mathbf{\hat{N}} \mathbf{a} }^2,
  \label{eq:cylinder_axis}
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
which is a homogeneous least square problem same as Equation~\ref{eq:plane_weighted_axis}, and can be solved in the same way.

Once obtaining the axis $\mathbf{a}$, we consider a plane $\mathscr{P}$ with normal $\mathbf{a}$ that passes through the origin, and notice the projection of the cylinder onto $\mathscr{P}$ should form a circle. 
Thus we can choose $\mathbf{c}$ and $r$ to be the circle that best fits the projected points $\{\text{Proj}_\mathbf{a}(\mathbf{P}_{i,:})\}_{i=1}^N$,
where $\text{Proj}_\mathbf{a}(\cdot)$ denotes the projection onto $\mathscr{P}$. This is exactly the same formulation as in the sphere case (Equation~\ref{eq:sphere_weighted}), and can thus be solved similarly. 

\vspace{-\baselineskip}
\paragraph{Cone.}
A cone is parameterized by $\mathbf{A} = (\mathbf{a}, \mathbf{c}, \theta)$ where $\mathbf{c} \in \mathbb{R}^3$ is the apex, $\mathbf{a} \in \mathbb{R}^3$ is a unit vector of the axis from the apex into the cone, and $\theta \in (0, \frac{\pi}{2})$ is the half angle. Then
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
  D^2_{\text{cone}}(\mathbf{p}, \mathbf{A})^2 = \left( \|\mathbf{v}\| \sin\left( \min\left( \left| \alpha - \theta \right|, \frac{\pi}{2}  \right) \right) \right)^2,
\end{equation}
where $\mathbf{v} = \mathbf{p} - \mathbf{c}, 
  \alpha = \arccos\left( \frac{\mathbf{a}^{\mathbf{T}}\mathbf{v}}{\|\mathbf{v}\|}\right)$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Similarly with the cylinder case, we use a multi-stage algorithm: first we estimate $\mathbf{a}$ and $\mathbf{c}$ separately, and then we estimate the half-angle $\theta$.

We utilize the fact that the apex $\mathbf{c}$ must be the intersection point of all tangent planes on the cone surface. Using the predicted point normals $\mathbf{\hat{N}}$, the multi-plane intersection problem is formulated as a least square similar with Equation~\ref{eq:sphere_weighted_center} by minimizing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
 \mathcal{E}_{\text{cone}}(\mathbf{c}; \mathbf{\hat{N}}) = \norm{ \text{diag}\left(\mathbf{w}\right) \left( \mathbf{\hat{N}} \mathbf{c} - \mathbf{y} \right) }^2,
\label{eq:cone_apex}
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where $\mathbf{y}_{i} = \mathbf{\hat{N}}_{i,:}^{\mathbf{T}}\mathbf{P}_{i,:}$.
To get the axis direction $\mathbf{a}$, observe that $\mathbf{a}$ should be the normal of the plane passing through all $\mathbf{N}_i$ if point $i$ belongs to the cone.
This is just a plane fitting problem, and we can compute $\mathbf{a}$ as the unit normal that minimizes Equation \ref{eq:plane_weighted}, where we replace $\mathbf{P}_{i,:}$ by $\mathbf{\hat{N}}_{i,:}$. 
We flip the sign of $\mathbf{a}$ if it is not going from $\mathbf{c}$ into the cone.
Finally, using the apex $\mathbf{c}$ and the axis $\mathbf{a}$, the half-angle $\theta$ is simply computed as a weighted average:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
  \theta = \textstyle\frac{1}{\sum_{i=1}^N \mathbf{w}_i} \sum_{i=1}^N \mathbf{w}_i \arccos \left|\mathbf{a}^\mathbf{T} \textstyle\frac{\mathbf{P}_{i,:}-\mathbf{c}}{\norm{\mathbf{P}_{i,:} - \mathbf{c}}}\right|.
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Loss Function}
\label{sec:loss_function}
\vspace{-3pt}

We define our loss function $\mathcal{L}$ as the sum of the following five terms without weights:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
  \mathcal{L} = \mathcal{L}_{\text{seg}} + \mathcal{L}_{\text{norm}} + \mathcal{L}_{\text{type}} + \mathcal{L}_{\text{res}} + \mathcal{L}_{\text{axis}}.
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Each loss term is described below for a single input shape.

\vspace{-\baselineskip}
\paragraph{Segmentation Loss.}
The primitive parameters can be more accurately estimated when the segmentation of the input point cloud is close to the ground truth. Thus, we minimize $(1 - \text{RIoU})$ for each pair of a ground truth primitive and its correspondence in the prediction:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
  \mathcal{L}_{\text{seg}} = \frac{1}{K} \sum_{k=1}^{K} \left( 1 - \text{RIoU}(\mathbf{W}_{:,k}, \mathbf{\hat{W}}_{:, k}) \right).
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{-\baselineskip}
\paragraph{Point Normal Angle Loss.}
For predicting the point normals $\mathbf{\hat{N}}$ accurately, we minimize the absolute cosine angle between ground truth and predicted normals:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
  \mathcal{L}_{\text{norm}} = \frac{1}{N} \sum_{i=1}^{N} \left( 1 - |\mathbf{N}_{i, :}^\mathbf{T}\mathbf{\hat{N}}_{i, :}| \right).
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The absolute value is taken since our predicted normals are unoriented.

\vspace{-\baselineskip}
\paragraph{Per-point Primitive Type Loss.}
We minimize cross entropy $H$ for the per-point primitive types $\mathbf{\hat{T}}$ (unassigned points are ignored):
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
  \mathcal{L}_{\text{type}} = \frac{1}{N} \sum_{i=1}^{N} \mathbb{1}(\mathbf{W}_{i,:} \neq \mathbf{0}) H(\mathbf{T}_{i,:}, \mathbf{\hat{T}}_{i,:}),
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where $\mathbb{1}(\cdot)$ is the indicator function.

\vspace{-\baselineskip}
\paragraph{Fitting Residual Loss.}
Most importantly, we minimize the expected squared distance between $\mathbf{S}_k$ and the predicted primitive $k$ parameterized by $\mathbf{\hat{A}}_{k}$ across all $k = 1,\ldots, K$:
% Since the input point cloud $\mathbf{P}$ may include noise, the fitting loss is measured not from the input point cloud but from the given ground truth surface segments $\{\mathbf{S_k}\}$:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
  \mathcal{L}_{\text{res}} &= \frac{1}{K} \sum_{k=1}^{K} \mathbb{E}_{\mathbf{p} \sim U(\mathbf{S}_k)} D^2_{\mathbf{t}_k}(\mathbf{p}, \mathbf{\hat{A}}_{k}),
\label{eq:residual_loss}
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where $\mathbf{p}\sim U(\mathbf{S})$ means $\mathbf{p}$ is sampled uniformly on the bounded surface $\mathbf{S}$ when taking the expectation, and $D^2_{l}(\mathbf{p}, \mathbf{\hat{A}})$ is the squared distance from $\mathbf{p}$ to a primitive of type $l$ with parameter $\mathbf{\hat A}$, as defined in Section~\ref{sec:model_estimation}. 
Note that every $\mathbf{S}_k$ is weighted equally in Equation~\ref{eq:residual_loss} regardless of its \emph{scale}, the surface area relative to the entire shape. This allows us to detect small primitives that can be missed by other unsupervised methods.

Note that in Equation \ref{eq:residual_loss}, we use the ground truth type $\mathbf{t}_k$ instead of inferring the predicted type based on $\mathbf{\hat{T}}$ and then properly weighted by $\mathbf{\hat{W}}$. 
We do this because coupling multiple predictions can make loss functions more complicated, resulting in unstable training.
At test time, however, the type of primitive $k$ is predicted as
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
\mathbf{\hat t}_k = \argmax_l \sum_{i=1}^N \mathbf{\hat{T}}_{i,l} \mathbf{\hat{W}}_{i,k}.
\label{eq:pred_per_primitive_type}
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{-\baselineskip}
\paragraph{Axis Angle Loss.}
Estimating plane normal and cylinder/cone axis using SVD can become numerically unstable when the predicted $\mathbf{\hat{W}}$ leads to degenerate cases, such as when the number of points with a nonzero weight is too small, or when the points with substantial weights form a narrow plane close to a line during plane normal estimation (Equation \ref{eq:plane_weighted_axis}). Thus, we regularize the axis parameters with a cosine angle loss:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
  \mathcal{L}_{\text{axis}} = \frac{1}{K} \sum_{k=1}^K \left(1 - \Theta_{\mathbf{t}_k}(\mathbf{A}_k, \mathbf{\hat{A}}_k) \right),
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where $\Theta_{t}(\mathbf{A}, \mathbf{\hat{A}})$ denotes $|\mathbf{a}^\mathbf{T}\mathbf{\hat{a}}|$ for plane (normal), cylinder (axis), and cone (axis), and $1$ for sphere (so the loss becomes zero).
%Depending on the primitive type, $\mathbf{a} \in \mathbf{A}$ means normal in planes, and axis in cylinders and cones. $\Theta_{t}(\mathbf{A}, \mathbf{\hat{A}}) = 0$ when $t$ is sphere.


\subsection{Implementation Details}
\label{sec:implementation_details}
\vspace{-3pt}
%In our implementation, we assume a fixed number $N$ of the input points for all input shapes.
In our implementation, we assume a fixed number $N$ \rev{of input points} for all shapes.
While the number of ground truth primitives varies across the input shapes, we choose an integer $K_\text{max}$ in prediction to fix the size the output membership matrix $\mathbf{\hat{W}} \in \mathbb{R}^{N\times K_\text{max}}$ so that $K_\text{max}$ is no less than the maximum primitive numbers in input shapes. After the Hungarian matching in Section~\ref{sec:primitives_reordering}, unmatched columns in $\mathbf{\hat{W}}$ are ignored in the loss computation.
At test time, we discard a predicted primitive $k$ if 
$
    \frac{\sum_{i=1}^N \mathbf{\hat{W}}_{i,k}}{N} > \epsilon_\text{discard}
    $,
%for a small constant threshold $\epsilon_{\text{discard}}$.
\rev{where $\epsilon_\text{discard}=0.005N$ for all experiments. This is just a rather arbitrary small threshold to weed out unused segments.}

When evaluating the expectation $\mathbb{E}_{\mathbf{p} \sim U(\mathbf{S}_k)}(\cdot)$ in Equation \ref{eq:residual_loss}, on-the-fly point sampling takes very long time in training.
%Hence the expectation is approximated as the average of the expression $(\cdot)$ evaluated at $M$ points on $\mathbf{S}_k$ that are sampled uniformly when preprocessing the data.
Hence the expectation is approximated as the average for $M$ points on $\mathbf{S}_k$ that are sampled uniformly when preprocessing the data.


==> sections/lingxiao_introduction.tex <==
% !TEX root = ../paper.tex

\section{Introduction}
\label{sec:introduction}
Recent advance in 3D scanning techniques made 3D data an important data modality in various industries, such as \AD{[FILL, and reverse engineering]}. \lingxiao{grammar: ``made data a data modality?''}
In parallel, large 3D data repositories~\cite{TurboSquid,GrabCad,TraceParts} are being created, opening opportunities for machine-learning-based 3D data analysis and manipulation.
However, most of the scanned data and the models in these repositories are represented as point clouds or meshes. Such \emph{rasterized} forms of 3D data limit our ability to geometrically manipulate it, due to the lack of structural information.\lingxiao{is rasterized the right term for 3D point cloud/meshes? I suppose we just mean low-level data. RANSAC paper uses ``digitized data/geometry''}
%\AD{We need to define what a "manipulation" means.}
For example, when editing a shape built of a number of geometric primitives (\lingxiao{what exactly do we mean by a primitive?}), the knowledge of the primitives can simplify the manipulation task, helping to produce a plausible result (Figure~\ref{fig:teaser}) \lingxiao{this sentence looks problematic: do we mean edit a point cloud sampled on a shape build from primitives? If we are editing a CAD file then we already know the primitives}. To address the absence of such structural information, in this work we propose an analogous \emph{raster-to-vector} conversion for 3D data - an approach for fitting a set of simple geometric primitives to a given 3D point cloud (\lingxiao{what does ``fitting'' mean? see the end of next paragraph}).
% PREVIOUS TEXT (Leaving here since I made quite a lot of changes): Recent 3D scanning techniques and large-scale 3D repositories widened opportunity for 3D geometric data manipulation. However, most of the scanned data and the models in online repositories are represented as point clouds or meshes, and such \emph{rasterized} forms of data limit the capability of manipulating the 3D shapes due to its lack of structural information. For example, when editing the shapes, it is necessary to know how the shape is composed of primitive parts. Thus, in this work, we consider a \emph{raster-to-vector} conversion problem in 3D, representing the input 3D shape with a set of simple geometric primitives.

Representing a low-level 3D data in the form of  point cloud or mesh with concise geometric abstractions is a long-established idea in computer vision, an idea that started out in the 1970s~\cite{Binford:1971,Marr:1978} and has been frequently studied by researchers till recent years~\cite{Tulsiani:2017,Zou:2017,Ganapathi:2018}. 
The majority of these work aimed at solving \emph{perceptual} learning tasks: the main focus was on roughly approximating the input shape with a set of bounding boxes and spheres. However, detailed geometric and semantic information is lost in such crude abstraction.
In contrast, we hope to extract richer information by predicting the precise types and parameters of the geometric primitives that best abstract the shape surface where the input low-level 3D data is sampled from, even with the presence of noise (as in the case of scanned data). This is commonly known as the \emph{primitive fitting} problem.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
  \centering
  \dummyfig{\columnwidth}{6cm}{Teaser}
  \caption{Teaser}
  \label{fig:teaser}
\vspace{-\baselineskip}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For over a decade, RANSAC-based methods~\cite{Schnabel:2007} have been the state of the art.
These methods typically first generate a set of candidates of primitives, where each candidate fits a minimal set of input points exactly, extract a best candidate based on heuristics that covers most points, assign close points to the candidate primitive, and then iterate.
The main drawback of the RANSAC-based approaches is in choosing good algorithm parameters - various thresholds values - in candidates selection and points assignment. For example, when choosing the maximal distance to assign a point to a candidate primitive, a value smaller than the noise level may lead to fragmented segmentation results, while a too large value will cause the algorithm to miss small primitives. 
This problem occurs not only when processing scanned data, but also when manipulating meshes in 3D repositories, since conversion of a CAD model into a mesh leads to loss of geometric information, \eg, cylinders are converted to multiple planes. \AD{mention that parameters must be chosen per-model, which also requires a lot of time?}

The above drawback motivated us to consider a \emph{supervised} learning framework. Given a large database of 3D shapes with ground truth geometric primitive information, we propose a neural-network-based framework taking sampled and, possibly, noisy input shapes as input, and producing a set of primitives in end-to-end fashion. \minhyuk{Rewrite: Directly adjusting RANSAC parameters in a neural network may require reinforcement learning techniques, due to the non-differentiable RANSAC procedure, which is known as notoriously difficult to train}. Directly regressing the primitive parameters is also not trivial, because of the different numbers of primitives in different shapes and the variety of primitive types. Moreover, small errors in the parameter space do not guarantee small fitting residuals. Hence, instead of these, we consider an approach of predicting per-sampled-point properties used to derive the primitive parameters, and is obtained by directly minimizing the fitting residual losses in the training.

Specifically, we introduce Supervised Primitive Fitting Network (SPFN) that takes a 3D shape represented as a point cloud, and estimates three types of per-point properties: a point to a primitive association, surface normal, and the type of the primitive the point belongs to. The types of primitives supported in SPFN are plane, sphere, cylinder, and cones, which are the most major components in CAD models. Given these per-point properties, we cluster points according to their primitives, and compute the primitive parameters of the most voted type using point positions and estimated normals. One of the advantages of our approach is that the parameter regression problem is transformed into three sub-problems: two are classification problems (membership, type), which have been extensively studied in various neural-network-based approaches \AD{or: "which have been shown particularly suitable to be solved using a neural-network-base approach"}, and the last is normal prediction, which was also proved as easy problem to address with a neural network~\cite{Bansal:2016,Guerrero:2018}. Moreover, the whole process of computing primitive parameters is made \emph{differentiable}, and thus during training, we can back-propagate the fitting residual loss through the layers predicting the per-point properties, even without any RNN-based iterative process.
%While input shapes have different numbers of primitives and primitive order is not consistent across shapes, we handle the problem by simply matching output and ground truth primitives using an external Hungarian algorithm.

To train and evaluate the proposed method, we collected a dataset of 3D mechanical component shapes, which we will release as a benchmark for primitive fitting algorithms. In our experiments, we demonstrate that our supervised approach outperforms a RANSAC-based approach~\cite{Schnabel:2007} with a big margin, even when training and testing the network using models from separate categories. Our method shows better fitting accuracy even when compared to running the RANSAC-based approach with much higher-resolution point clouds.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-0.5\baselineskip}
\paragraph{Key contributions}
\begin{itemize}
  \setlength\itemsep{-0.1em}
  \item End-to-end supervised NN framework...?
  \item Benchmark
\end{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


